Searching Personal Collections

This article describes the history of information retrieval on personal document collections.

==> front.tex <==
% This front matter template includes only the information you need to
% give us. We will take care of the rest of the front matter.

\title{Advanced Topics for Information Retrieval}
\author{Omar Alonso, Ricardo Baeza-Yates}

\maketitle

% Dediction, if you have one.

\tableofcontents


